Central-limit approach to risk-aware Markov decision processes

Whereas classical Markov decision processes maximize the expected reward, we consider minimizing the risk. We propose to evaluate the risk associated to a given policy over a long-enough time horizon with the help of a central limit theorem. The proposed approach works whether the transition probabilities are known or not. We also provide a gradient-based policy improvement algorithm that converges to a local optimum of the risk objective.

==> intro.tex <==
%\documentclass[twoside]{article}
%\usepackage{aistats2016}
%
%% If your paper is accepted, change the options for the package
%% aistats2016 as follows:
%%
%%\usepackage[accepted]{aistats2016}
%%
%% This option will print headings for the title of your paper and
%% headings for the authors names, plus a copyright note at the end of
%% the first column of the first page.
%
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
%\usepackage{bibentry}
%
%\usepackage{import}
%
%\begin{document}
%
%% If your paper is accepted and the title of your paper is very long,
%% the style will print as headings an error message. Use the following
%% command to supply a shorter title of your paper so that it can be
%% used as headings.
%%
%%\runningtitle{I use this title instead because the last one was very long}
%
%% If your paper is accepted and the number of authors is large, the
%% style will print as headings an error message. Use the following
%% command to supply a shorter version of the authors names so that
%% they can be used as headings (for example, use only the surnames)
%%
%%\runningauthor{Surname 1, Surname 2, Surname 3, ...., Surname n}
%
%\twocolumn[
%
%\aistatstitle{Instructions for paper submissions to AISTATS 2016}
%
%\aistatsauthor{ Anonymous Author 1 \And Anonymous Author 2 \And Anonymous Author 3 }
%
%\aistatsaddress{ Unknown Institution 1 \And Unknown Institution 2 \And Unknown Institution 3 } ]




Markov Decision Processes (MDPs) are essential models for stochastic sequential decision making problems \citep[e.g.,][]{puterman2014markov,bertsekas1995dynamic,sutton1998reinforcement}. Classical MDPs are concerned with the expected performance criteria. However, in many practical problems, risk-neutral objectives may not be appropriate \citep[cf.][Example 1]{ruszczynski2010risk}.

Risk aware decision making is prevalent in the financial mathematics and optimization literature  \citep[e.g.,][]{artzner2002coherent,rockafellar2007coherent}, but limited to single-stage decisions. Risk-awareness has been adopted in multi-stage or sequential decision problems more recently. A chance-constrained formulation for MDPs with uncertain parameters has been discussed in \citep{delage2010percentile}. A criteria of maximizing
the probability of achieving a pre-determined target performance has been analyzed in \citep{xu2011probabilistic}. In \citep{ruszczynski2010risk}, Markov risk measure is introduced and a corresponding risk-averse policy iteration method is developed. \citet{osogami2012robustness} uncovers relations between robust MDPs and risk-sensitive MDPs. A mean-variance optimization problem for MDPs is addressed in \citep{guo2012mean}. In terms of computational convenience, actor-critic algorithms for optimizing variance-related risk measures in both discounted and average reward MDPs have been proposed in \citep{prashanth2013actor}. Mean and conditional value-at-risk optimization problem in MDPs is solved by policy gradient and actor-critic algorithms in \citep{chow2014algorithms}. A unified policy gradient approach is proposed in \citep{tamar2015policy} to seek optimal strategy in MDPs with the whole class of coherent risk measures.
Risk-aversion in multiarmed bandit problems is studied in \citep{yu2013sample}, where algorithms are proposed with PAC guarantees for best arm identification.
% However, we consider the approach proposed in \cite{yu2013sample} is quite restrictive. First, in general, the rewards $r_i$, $i = 1,\cdots,T$ generated by following a Markov chain induced by a policy are usually dependent. Secondly, as $T\rightarrow\infty$, the method proposed in \cite{yu2013sample} is intractable. Specifically, the density estimation of $r_1+\cdots+r_\tau$ by convolution becomes computationally hard.

In this work, we use the notion of monetary value of risk and apply it to MDPs.
Computing this risk associated with a sequence of decision using the defintion and first principles is intractable.
However, we show that this computation is made tractable by using
a central limit theorem for Markov chains
\citep{jones2004markov,kontoyiannis2003spectral,glynn1996liapounov}.
For a moderately long time horizon $T$ and a fixed policy $\pi$, we are thus able to evaluate the risk associated with following policy $\pi$ over $T$ time steps.
% This risk can be expressed as a function of the distribution of cumulative reward.
Specifically, our first contributions are policy evaluation algorithms whether the transition probability matrix induced by $\pi$ is known or not. Under mild conditions, we provide high-probability error bounds for the evaluation.
It is important to note that our risk measure is very different from that analyzed in \citep{ruszczynski2010risk}, which uses multiple iterations of one-step risk functions. Our risk measure emphasizes the statistical properties the reward accumulated over multiple time steps: it is similar to that used in \citep{yu2013sample} in the context of bandit problems.

For a fixed risk measure $\rho$, and a space of policies that is parametrized by $\theta$, we propose a policy improvement algorithm 
that converges in finite iterations, under certain assumptions,
to a locally optimal policy.
This approach updates the parameter $\theta$ in the direction of gradient of the risk measure.
Compared to the previous work, our proposed method does not explicitly approximate the value function. Therefore, it does not have approximation error due to the selection of value function approximator. 

\citet{tamar2015policy} defined two types of coherent risk measures: static and time-consistent dynamic risk measures. The static coherent risk measure is a function $\rho:\mathcal{Y}\rightarrow\mathbb{R}$ that maps an uncertain outcome $\mathcal{Y}$ to the extended real line $\mathbb{R}\cup\{+\infty,-\infty\}$ satisfying convexity, monotonicity, translation invariance and positive homogeneity properties \citep[cf.][]{artzner2002coherent}. The dynamic risk measure has the following structure: for $T$-length horizon MDP and policy $\pi$, the dynamic risk measure $\rho_T$ is defined by $$\rho_T=r(x_0^\pi)+\gamma\rho(r(x_1^\pi)+\cdots+\gamma\rho(c(x_{T-1}^\pi)+\gamma\rho(r(x_T^\pi)))),$$
where $r(x)$ is a state dependent reward, $\gamma<1$ and $\rho$ is a Markov risk measure, i.e., the evaluation of each static coherent risk measure $\rho$ is not allowed to depend on the whole past \citep[e.g.,][]{ruszczynski2010risk}.

Previous work \citep[e.g.,][]{delage2010percentile,xu2011probabilistic,guo2012mean,chow2014algorithms,prashanth2013actor} have focused on specific risk measures. Even though we deal with the static risk measure (those are defined by the accumulative reward), we remark that static risk measures considered in this paper are not necessary coherent. One typical example is value-at-risk \citep{duffie1997overview}, which is not a coherent risk measure.



